HyperBlocker: Accelerating Rule-based Blocking in Entity Resolution using GPUs

This paper studies rule-based blocking in Entity Resolution (ER). We propose HyperBlocker, a GPU-accelerated system for blocking in ER. As opposed to previous blocking algorithms and parallel blocking solvers, HyperBlocker employs a pipelined architecture to overlap data transfer and GPU operations. It generates a dataaware and rule-aware execution plan on CPUs, for specifying how rules are evaluated, and develops a number of hardware-aware optimizations to achieve massive parallelism on GPUs. Using reallife datasets, we show that HyperBlocker is at least 6.8x and 9.1x faster than prior CPU-powered distributed systems and GPU-based ER solvers, respectively. Better still, by combining HyperBlocker with the state-of-the-art ER matcher, we can speed up the overall ER process by at least 30% with comparable accuracy.

==> response.tex <==
\twocolumn
\balance
\pagestyle{plain}


\section*{Response to Reviews (Shepherd Submission \#442 $\ra$ \#655)}
\vspace{2ex}

\ni
Dear Meta Reviewer and Referees:

\vspace{1ex}
We would like to thank the referees for their thorough reading
of our paper and for their helpful comments.
We have substantially revised the paper
following the Referees' suggestions.
For the convenience of Referees, changes to the paper 
are color-coded in {\color{blue} blue}. \looseness=-1

%\reviseMeta{purple}, \reviseOne{blue}, \reviseTwo{red}, \reviseThree{brown}
%in response to the suggestions of Meta Reviewer, Referees~1, 2, and 3, respectively.


%\vspace{0.6ex}
%We would like to thank Referees for helpful comments.

\vspace{0.6ex}
Below please find our responses to the reviews.



\vspace{2ex}
\hrule
\vspace{0.6ex}
\ni
\noindent {\bf Response to the comments of the Meta Reviewer.}

\vspace{1.2ex} \noindent
{\em  {\bf [Q3]}
Please look carefully at the reviews. However, below are the main reviewers' comments to be addressed.

W1: I was hoping for a clear explanation of novelty and originality especially since predicate ordering is a classical RDBMS problem. However, I couldn't quite understand the new paragraph in section 7. It sounds like this paper might be solving a simpler problem than RDBMS predicate ordering, making me even more concerned about novelty with respect to this classical work. Then on page 5, the unique challenges don't sound unique to me. For example, deciding which predicate to evaluate first so that the rule fails early is a common strategy for conjunctive predicates, including those in RDMBSs.

W2: The new example in the introduction explains shared memory vs shared nothing in general, but I was hoping for a specific example and explanation in the context of blocking. How does the parallelism afforded by GPUs benefit blocking specifically?

}

\vs
\noindent
{\bf [A]}
We have
revised the paper to address all revision items.

In addition,
we have simplified some discussion and moved some experimental results to the online full version~\cite{full}, to make room
for the newly added examples and discussion.

% Response to R4
\vspace{2ex} \hrule \vspace{0.6ex}
\noindent {\bf Response to the comments of Referee \#4.}

\vspace{1.2ex} \noindent
{\em {\bf [W2-1]}
Does COrder partition the dataset based on the equality predicates or does it only prioritize them? If it only prioritizes them, then divergence is still an issue (and traditional partitioning-based techniques wouldn't have this issue).}

\vs
\noindent
{\bf [A]} 
Thanks! We have clarified the following.

\sstab 
(1) For a fair comparison,
we have remarked in pp.~11 that we applied the same partitioning strategy (Section~\ref{subsec:GPUs}) for all orders.

\sstab 
(2) In our data partitioning strategy (Section~\ref{subsec:GPUs}, pp.~8-9),
the hash functions are constructed based on the root node $N_0$ and its children nodes.
In this way,
the predicates that we adopt for data partitioning are indeed those predicates prioritized by the execution plan $\mathcal{T}$,
in order to alleviate the issue of divergence as suggested.



\vspace{1.2ex} \noindent
{\em {\bf [W2-2]}
Similarly, for SOrder, after evaluating the selective predicates, does it reorganize the data so that there are not threads working on filtered-out data?}


\vs
\noindent
{\bf [A]} Thanks!  We will not reorganize the data in blocking,
since the evaluation of each tuple pair $(t_1, t_2)$ is an \emph{independent} task (pp.~7)
and we process them one by one. 
Moreover, even if $(t_1, t_2)$ fails to satisfy a selective predicate $p$,
it does not necessarily mean that $(t_1, t_2)$ is not a match and the thread can stop working on it.
This is because there maybe another rule $\varphi: X \ra l$ in $\Delta$ such that $p \not \in X$ and $h(t_1, t_2) \models X$.
In this case, 
the thread will still work on $(t_1, t_2)$ for checking other rules in $\Delta$ (even after it finds $h(t_1, t_2)\not \models p$),
unless $(t_1, t_2)$ fails to satisfy \emph{all} blocking rules in $\Delta$.
Nevertheless,
we employ the tree structure and bitmaps, to effectively handle the
disjunction logic behind blocking and to avoid repeated evaluations (pp.~7).
\looseness=-1


\vspace{1.2ex} \noindent
{\em {\bf [W2-3]}
It may worth considering extending (potentially as a future work) HyperBlocker to decide when to materialize the current (partial) evaluation results before proceeding with the rest of the evaluation. For example, if there is an expected 70\% rejected inputs after the 5th predicate, it may worth writing out the qualifying inputs, and rereading them in a second evaluation "round" that only runs the 6th predicate onwards on the 30\% qualifying inputs, to avoid divergence.
}

\vs
\noindent
{\bf [A]} 
Thanks! We have added this future work as suggested (pp.~12).





\eat{
2. In SOrder, we avoid data reorganization by using tree structure of execution plan~(pp \tbf) and  a bitmap~(pp \tbf) to efficiently track and reuse computations. 
This approach ensures that threads focus only on relevant data, minimizing unnecessary work without the need to rearrange the dataset.

  
3. Thanks for the suggestion! 
We have added this in future work.

We initially considered multi-query optimization (MQO)\cite{MQO}, which materializes common sub-expressions, but ultimately did not adopt it for two reasons:
(1) MQO focuses on reusing shared subexpressions to reduce the computational cost, while our matching order optimization (Section\ref{sec-plan}) improves efficiency by optimizing the sequence of predicate evaluations. These two methods might conflict, as MQO might push down selective or costly predicates, causing performance degradation~(\ie disrupt the origin order). Therefore, we prioritize matching order and selectively apply computation reuse using a bitmap;
(2) GPUs have limited memory compared to CPUs, and materializing intermediate results can quickly exhaust this capacity.
In summary, integrating MQO with matching order optimization merits deeper discussion.

}


\vspace{1.2ex} \noindent
{\em {\bf [D4]}
Then, maybe it would be nice to add a discussion on how to select good parameter values during runtime, if the results are sensitive to the parameters and the parameters are sensitive to the inputs.
}

\vs
\noindent
{\bf [A]} 
Thanks! We have remarked in pp.~9-10
that
the default parameters,
are best-tuned 
via \emph{gird search}~\cite{jimenez2008finding}.
Intuitively, gird search is a practical method for
systematically exploring the parameter space to get the set of parameters that results in the best performance.

\vspace{1.6ex}
Many thanks for your support and helpful suggestions!

% Response to R7
\vspace{2ex} \hrule \vspace{0.6ex}
\noindent {\bf Response to the comments of Referee \#7.}





\vspace{1.2ex} \noindent
{\em {\bf [W1]}
I was hoping for a clear explanation of novelty and originality especially since predicate ordering is a classical RDBMS problem. However, I couldn't quite understand the new paragraph in section 7. It sounds like this paper might be solving a simpler problem than RDBMS predicate ordering, making me even more concerned about novelty with respect to this classical work. Then on page 5, the unique challenges don't sound unique to me. For example, deciding which predicate to evaluate first so that the rule fails early is a common strategy for conjunctive predicates, including those in RDMBSs.
}

\vs
\noindent
{\bf [A]} 
Thanks!
We have made the following major changes:

\sstab
(1) We have clarified in pp.~3 that since a precondition is a conjunction of predicates,
rule-based blocking is in \emph{Disjunctive normal form} (DNF), \ie 
it is to evaluate a disjunction of conjunctions.
Moreover, rule-based blocking supports both equality and similarity comparisons.
In particular,
sophisticated similarity measures like ML models can also be used for similarity comparisons~\cite{REE-discovery,rock}.


\sstab 
(2) We have discussed the use of the existing optimizers of DBMS to tackle rule-based blocking (pp.~5).
As remarked in~\cite{preedet,rock},
blocking with a set of \MDs can be implemented in a single DNF SQL query (\ie an {\tt OR} of 
{\tt ANDs}),
where similarity predicates in \MDs are re-written as user-defined functions (UFDs).
This, however, may not work well, for several reasons.
\eat{(a) The compilation/translation of UDFs may introduce significant overheads.
As evidenced in~\cite{rock},
even modern engines like \kw{SparkSQL}~\cite{sparksql}and \kw{Presto}~\cite{prestosql} cannot finish the execution in
one day when SQLs are embedded with complicated UDFs.}
(a) The mixture of relational operators and UDFs poses serious challenges to an optimizer~\cite{rheinlander2017optimization}.
It may lack ``the information needed to decide whether they can be reordered with
relational operators and other UDFs''~\cite{hueske2013peeking}
and worse still,
it is hard to  accurately estimate the runtime performance of UDFs~\cite{rheinlander2017optimization}.
(b) Using {\tt OR} operators in {\tt WHERE} clauses can be inefficient since it can force the database to perform a full table scan to find matching tuples~\cite{badOR}. %\looseness=-1
(c) Similar to~\cite{li2023selection}, 
if a tuple pair fails to satisfy prior predicates in a blocking rule, the remaining evaluation of this rule can be bypassed directly.
While this is undeniably obvious, ``many approaches have not leveraged it effectively''~\cite{li2023selection}.


\sstab 
(3)
To justify the issues of existing optimizers  mentioned above,
we have conducted an additional test in~\cite{full}
using \kw{PostgreSQL}~\cite{postgresql}, a popular DBMS, on different queries,
by (a) specifying similarity predicates in different orders 
and (b) evaluating SQLs with or without {\tt OR} operators.
Using \kw{PostgreSQL}'s {\tt EXPLAIN} feature, we find the following: 
(a) Although \kw{PostgreSQL} may prioritize equality, 
it does not optimize the order of similarity predicates well,
\eg it evaluates similarity predicates simply as specified in the SQLs, leading to 20\% slowdown on average.
(b) When handling {\tt OR} operators, \kw{PostgreSQL} may perform sequential scans with nested loops, without utilizing the hash index.
These findings highlight the need for designated optimization for rule-based blocking,
where we have to handle similarity comparisons and DNF evaluation efficiently.


\sstab
(3) We have revised the discussion in Section~\ref{sec:related-work} (pp.~12) accordingly 
and clarified our differences:
(a) EPG optimizes the execution, no matter what comparisons (\eg equality or similarity) are adopted,
while many DBMS optimizers struggle when similarity comparisons are encoded as UDFs, \eg SQL Server~\cite{sql_server} restricts UDFs to a single thread, and PostgreSQL~\cite{postgresql} treats UDFs as black boxes. 
This said, EPG solves a more specialized
problem, beyond general query optimization, for supporting arbitrary comparisons.
(b) It is hard for most optimizers to accurately estimate the runtime performance of UDFs~\cite{rheinlander2017optimization}, which may depend on specific measures, thresholds, and data (\ie data-awareness). At the same time, we consider both the time and the selectivity of predicates, using a learned and LSH-based model for accurate estimation. %beyond type limitations.
(c) EPG employs tree structures and bitmaps, to effectively handle the disjunction logic behind blocking and to reuse computation,
while traditional DBMS may be forced to perform a full scan when evaluating {\tt OR} operations.
(d) EPG also produces a data partitioning scheme based on the execution tree as a by-product, to coordinate across multiple GPUs.
%ensuring better utilization and reducing computation.


\sstab
(4) We have conducted supplementary experiments in~\cite{full}, by
replacing the execution plan generated by EPG in \Hyper with alternative plans generated by other systems
and report the runtime of the resulting blocking.
Specifically,
we compared the plans from the following systems:
(1) \kw{PostgreSQL}~\cite{postgresql}, a widely adopted DBMS;
we extract its execution plan using the {\tt EXPLAIN} feature.
(2) \kw{TupleX}~\cite{tuplex},
which is designed for Python-based UDFs optimization for data processing;
we format the query logic in Python and extract the plan from the log file.
As shown there,
the execution plan generated by EPG consistently beats the one generated by \kw{PostgreSQL}  by $114\times$ (resp. \kw{TupleX} by 38.5\%) on average on all datasets.

\sstab
(5) We have left the further investigation of whether EPG
and traditional optimizers can complement/enhance each other as an interesting future topic (pp.~12).
We have also carefully proofread the paper
to position our novelty better accordingly.



\eat{ 
EPG of \Hyper solves a more specialized
query optimization problem than general SQL query, as it focuses on
blocking rules that is in  DNF and with UDFs.
While, our evaluations show that PostgreSQL, an advanced open source DBMS, fails to handle UDFs and DNF efficiency~(see~\cite{full}).


This is mainly because existing DBMS optimizers~\cite{postgresql,sql_server,MQO,klonatos2014building,shaikhha2016architect,simjoin_order} either myopically focus on optimizing common predicates (\eg joins, filtering) without addressing UDF optimization~\cite{postgresql,sql_server,MQO,klonatos2014building,shaikhha2016architect}, or they limit their analysis to UDF logic, overlooking the impact of data distribution~\cite{simjoin_order} on UDF execution costs. While there has been work on analytics pipelines with Python UDFs~\cite{tuplex}, 
however, the key issue of selecting an appropriate order that accounts for data distribution remains unresolved~(see \cite{full}).


We have accordingly expanded the related work~\ref{sec:related-work}~(pp.~12).
to discuss key differences between existing query optimizer and EPG~(pp~5).

A case study on query plan generation and an experimental comparison between existing DBMS optimizers and state-of-the-art UDF optimizers are presented in our full version~\cite{full}.
}

%The query optimizer in existing DBMS has certain limitations that make it difficult to efficiently handle rule-based blocking.

\eat{
Prior methods for query optimization in RDBMSs, 
can be broadly categorized into optimizations for standard SQL queries~\cite{MQO, kathuria2017efficient, neo, li2015efficient, larson2007cardinality, moerkotte2006building} 
and those involving User-Defined Functions (UDFs) - custom functions created by users to express more complex predicates~\cite{udf1,rheinlander2017optimization}. 
Since \MDs extend equivalence rules not only to traditional SQL but also to more complex rules involving UDFs~\cite{rock}, 
and given that many standard optimizers struggle to optimize queries with UDFs — for example, 
UDFs in SQL Server can only be executed on a single thread~\cite{sql_server} and PostgreSQL treats UDFs as black box — 
this paper focuses on optimizing execution plans that involve UDFs.
}

\eat{
At first glance, existing optimizers might seem applicable to our problem. 
However, as noted in Section~\ref{sec-plan} and demonstrated in our experiments in the full version~\cite{full}, 
these methods struggle with optimizing blocking rules due to the unpredictable costs of UDFs 
and the complexity of handling multiple blocking rules.

In our full version~\cite{full}, 
we tested our proposed execution plan against two state-of-the-art optimizers: \kw{PostgreSQL}, an open-source DBMS, 
and \kw{TupleX}, a UDFs-based optimizer. 
Our optimizer consistently outperformed both~(see full version~\cite{full}).

The reason lies in the limitations of existing query optimizers, 
which rely heavily on accurate statistics and cost models. 
With UDFs, estimating selectivity becomes significantly more challenging due to the specific function, 
threshold, and data distributions—factors that are difficult to estimate, 
making it hard to adapt existing cost models effectively.

As a result, prior work often treats UDFs as black boxes, 
hindering optimizations across UDFs~\cite{UDF_tutorial}, 
or merely analyzes UDF logic to enable operation reordering or operator fusion~\cite{tupleware,simjoin_order,tuplex}. 
When UDFs share the same logic but operate on different data, 
or when multiple blocking rules are connected by "OR" logic, these methods tend to perform poorly.
}



\eat{
Seemly, the prior optimizer transferrable for our problem.
However, as noted in Section~\ref{sec-plan} and experiment in our full version~\cite{full},
these method do not work well for optimizing blocking rules as hardly perdictable cost of UDFs and collaborating multiple blocking rules.

In full version~\cite{full}, we did test our proposed execution plan method against two optimizer:
\kw{PostgreSQL} and \kw{TupleX}, the first one is SOTA open source DBMS while the latter is SOTA UDFs-based optimizer.
Our optimizer consistenly outperforms them.

The reason is that 
existing query optimizers rely on accurate statistics about data distribution and cost models.
However, with UDFs, estimating selectivity becomes significantly more challenging because it depends on the specific function, 
threshold, and data distributions—factors that are not straightforward to estimate,
making it difficult to adapt existing cost models.

Prior work either treats UDFs as black boxes, preventing optimizations across UDFs~\cite{UDF_tutorial}, 
or merely analyzes the logic of UDFs to enable operation reordering or operator fusion~\cite{tupleware,simjoin_order,tuplex}.
When the rule consisting of UDFs with shared the same logic but run on different data, 
or there are multiple rules connected via OR logic, these method do not perform well.
}


\eat{
%We aware of that execution plan depends on both computational cost of UDFs and the effectiveness of UDFs~(\ie filtering ability).

Tupleware~\cite{tupleware} provides a UDF-aware compiler that can apply some optimization to black-box UDFs,
however, it lacks support for None-valued in UDFs~\cite{tuplex}. 
Tuplex~\cite{tuplex} and Yasin et al.~\cite{simjoin_order} optimize UDF placement by analyzing abstract syntax trees or query trees, pushing UDFs up and down the joins~(\eg push filters to the start of workflow). 
However, they are not aware of the importance of data that might impact query performance, which could be crucial in designing a more effective execution plan.
%As reported in \cite{or}, which analyzes execution plans in PostgreSQL, "OR" can hinder optimization by preventing  index usage, 
%leading to sequential full table scans. 
}

\eat{
Compared to prior work~(pp \tbf), EPG optimizes \MDs with UDFs differently in several key aspects. 
Firstly, the strategy and cost model for building execution plans are significantly different. 
Instead of treating UDFs as black boxes or merely analyzing their logic, our cost model considers both the elapsed time and the filtering ability of predicates (including UDFs). 
Based on this, we devised a light-weight learned model-based and LSH-based cost model to order predicates, 
allowing for quick and accurate measurement of execution costs.
Secondly, the strategy for processing multiple rules are different.
Rule-based blocking often involves processing multiple rules, 
each connected by an \emph{OR} clause. 
DBMS optimizers may struggle to handle "OR" conditions. 
The execution tree and bitmap for multiple \MDs collaborate efficiently to apply predicates (including UDFs).
across different \MDs while maintaining the utility of indexes.
Thirdly, without partitioning, 
executing the plan remains costly for our problem, as it underutilizes multiple GPUs. 
To improve performance, we developed a data partitioning algorithm based on the execution plan. 
This algorithm prioritizes "high-priority" columns to generate partition keys, 
effectively reducing redundant computations.
}


%Precisely evaluating these factors is challenging, and the high overhead of building such a model would be unacceptable for our problem. Therefore, we devised a lightweight, learned model-based and LSH-based cost model to order predicates, enabling quick and accurate measurement of execution costs.


\eat{
Compare to prior work~(pp \tbf),
EPG optimizes \MDs with UDFs differently in several key aspects. 
Firstly, the strategy and cost model for building execution plans differ significantly. 
Our cost model considers both the elapsed time and the filtering ability of predicates (including UDFs) instead of treading them as a black box or merely analyzing the logic UFDs. 
Precisely evaluating these two factors is challenging, and the high overhead of building such a model is not acceptable for our problem. 
Therefore, we devised a lightweight learned model-based and LSH-based cost model to order predicates, allowing for quick and accurate measurement of execution costs.
Secondly,  the strategy for processing multiple rules is different.
Rule-based blocking often involves processing multiple rules, 
each connected by an \emph{OR} clause. 
DBMS optimizers may struggle to handle "OR" conditions. 

The execution tree and bitmap for multiple \MDs collaborate efficiently to apply predicates (including UDFs) 
across different \MDs while maintaining the utility of indexes.
Thirdly, without partitioning, the elapsed time for executing the plan remains expensive for our problem, as it leaves multiple GPUs underutilized. 
To further enhance performance, we developed a data partitioning algorithm based on the execution plan. 
This algorithm uses "high-priority" columns to generate partition keys, 
effectively reducing redundant computation.
}






\vspace{1.2ex} \noindent
{\em {\bf [W2]}
The new example in the introduction explains shared memory vs shared nothing in general, but I was hoping for a specific example and explanation in the context of blocking. How does the parallelism afforded by GPUs benefit blocking specifically?
}

\vs
\noindent
{\bf [A]} Thanks! As suggested,
we have revised the example specifically in the context of blocking (Figure~\ref{fig:shared_memory_vs_shared_nothing}, pp.~2),
where 
a blocker typically conducts pairwise comparisons on all pairs of tuples to obtain candidate matches (Figure~\ref{fig:shared_memory_vs_shared_nothing}(a)). 
In a shared-nothing architecture, %(adopted by many  MapReduce-based systems), 
data is partitioned and spread across a set of processing units.
Each unit independently blocks data using its local memory, which may lead to skewed partitions/computations and rising communication costs,
\eg in Figure~\ref{fig:shared_memory_vs_shared_nothing}(c),
the first unit is assigned more tuples than the second one and worse still,
two tuples that both refer to entity 1 are distributed to different partitions.
To avoid missing this match,
the second unit has to visit its local memory (Stp. 1) and transfer its data to the first unit (Stp. 2).
Then the first unit buffers the data (Stp. 3) and finally, conducts comparison locally (Stp. 4 \& 5). 
The shared memory architecture (Figure~\ref{fig:shared_memory_vs_shared_nothing}(b)) is the opposite: all data is accessible from all processing units,
allowing for efficient data sharing, collaboration between processing units and dynamic workload scheduling,
\eg the two tuples referred to entity 1 can be directly accessed by both units in Figure~\ref{fig:shared_memory_vs_shared_nothing}(b) (Stp. 1 \& 2).


\eat{
Given that blocking is a computationally intensive task~\cite{}, the parallelism of GPUs benefits it by enabling the simultaneous processing of multiple data blocks, without the data transfer costs caused by mismatches between entities. Unlike CPUs, GPUs handle large datasets in parallel, reducing bottlenecks. Additionally, we've re-plotted the picture in the example to better illustrate this concept.
}


\vspace{1.6ex}
Many thanks for helping us improve the paper!

% Response to R4
\vspace{2ex} \hrule \vspace{0.6ex}
\noindent {\bf Response to the comments of Referee \#8.}

\vspace{1.2ex} \noindent
{\em {\bf [Q3]}
IMHO the authors did a great job to further improve the paper, taking the feedback of the reviewers into account.

This will be a great addition to PVLDB.}

\vs
\noindent
{\bf [A]} 
Many thanks for supporting this work!



\newpage
\nobalance
